LookOut on Time-Evolving Graphs: Succinctly Explaining Anomalies from Any Detector

Why is a given node in a time-evolving graph ($t$-graph) marked as an anomaly by an off-the-shelf detection algorithm? Is it because of the number of its outgoing or incoming edges, or their timings? How can we best convince a human analyst that the node is anomalous? Our work aims to provide succinct, interpretable, and simple explanations of anomalous behavior in $t$-graphs (communications, IP-IP interactions, etc.) while respecting the limited attention of human analysts. Specifically, we extract key features from such graphs, and propose to output a few pair (scatter) plots from this feature space which "best" explain known anomalies. To this end, our work has four main contributions: (a) problem formulation: we introduce an "analyst-friendly" problem formulation for explaining anomalies via pair plots, (b) explanation algorithm: we propose a plot-selection objective and the LookOut algorithm to approximate it with optimality guarantees, (c) generality: our explanation algorithm is both domain- and detector-agnostic, and (d) scalability: we show that LookOut scales linearly on the number of edges of the input graph. Our experiments show that LookOut performs near-ideally in terms of maximizing explanation objective on several real datasets including Enron e-mail and DBLP coauthorship. Furthermore, LookOut produces fast, visually interpretable and intuitive results in explaining "ground-truth" anomalies from Enron, DBLP and LBNL (computer network) data.

==> 020background-christos.tex <==
Angiuli+: ====================
Drawbacks:
- scalability: O( h**(d-1) ) where d is the number of attributes,
   and $h$ is the number of base conditions
- non-verbal (gives explanation-property pairs, where
- succinct: it tries to explain all outliers.

Intuitively: find patches of address space, and a corresponding attribute $a$,
where the distribution of outliers on attribute $a$
is statisticall diff. from the inliers

Ie.: expects 
- records with $d$ attributes (num/cat)
- a set of records labeled as 'outliers'
- and the rest, 'inliers'
Returns:
- set of pairs of [patches (explanation) and property]

Dang, Assent, Ng, etc ==================
given $D$-dim points (in- and out-liers), project them to lower dim, 
so that the distances between inliers are small, 
and the distances across in-/out-liers, are large.

- scalability: complexity could approach O(n**2), for high $D$
  (no wall-clock times reported)
- non-verbal



==> 031discussion.tex <==
\subsection{Discussion}
We conclude our algorithm description by emphasizing a few points and the logic behind several design choices.

\noindent \textit{1. How do we define ``anomaly?''} %— we don’t care, whatever the blackbox says
This work focuses on the explanation of {\em given}, pre-identified anomalies.
Simply, we are oblivious to what constitutes an anomaly, and how the anomalies were detected -- in practice, several different types of anomalies can exist, including statistical, distance and model-based anomalies.

\vspace{1mm}

\noindent \textit{2. Why pair plots?} 
Using pair plots for justification is an essential, concious choice we make for several reasons:
(1) scatterplots are easy to look at and quickly interpret,
(2) they are universal and non-verbal, that is, we need not use language to convey the anomalousness of points, and
(3) they show where the anomalies lie {\em relative to the normal points}---the contrastive visualization of points is more convincing than stand-alone rules.

\vspace{1mm}

\noindent \textit{3. How do we choose the budget?} We designed our explanation objective to be budget-oriented, and let the budget be specified by the analyst. In general, humans have a working memory of size ``seven, plus or minus two'' \cite{miller1956mns}.


%4. Why these features? Are there more? — as we show in the experiments, we find that 
%one can extend, we use the listed 20 to show proof of concept.

